Quasi Markov Chain Monte Carlo Methods

Quasi-Monte Carlo (QMC) methods for estimating integrals are attractive since the resulting estimators typically converge at a faster rate than pseudo-random Monte Carlo. However, they can be difficult to set up on arbitrary posterior densities within the Bayesian framework, in particular for inverse problems. We introduce a general parallel Markov chain Monte Carlo (MCMC) framework, for which we prove a law of large numbers and a central limit theorem. In that context, non-reversible transitions are investigated. We then extend this approach to the use of adaptive kernels and state conditions, under which ergodicity holds. As a further extension, an importance sampling estimator is derived, for which asymptotic unbiasedness is proven. We consider the use of completely uniformly distributed (CUD) numbers within the above mentioned algorithms, which leads to a general parallel quasi-MCMC (QMCMC) methodology. We prove consistency of the resulting estimators and demonstrate numerically that this approach scales close to $n^{-2}$ as we increase parallelisation, instead of the usual $n^{-1}$ that is typical of standard MCMC algorithms. In practical statistical models we observe multiple orders of magnitude improvement compared with pseudo-random methods.

==> containment_trialproof.tex <==
\begin{assumption}
\label{assumption:continuity_measure}
The density of the target is continuous and positive.\\
\end{assumption}

\begin{assumption}[Integrability condition]
\label{assumption:intgrability_dim_adapt}
Let us assume that for sufficiently small $s>0$,
\begin{align*}
\int_{\mathbb{R}^{d}} \pi(\vec{x})^{1-s}\mathrm{d}\vec{x}< \infty.
\end{align*}
\end{assumption}

\begin{assumption}[Tail convergence condition]
\label{assumption:tail_convergence_dim_adapt}
For any sequence $(\vec{x}_j)_j \subset \mathbb{R}^d$
with $\lim_{n\rightarrow \infty}\vec{x}_n = +\infty$, there is a subsequence
$(\tilde{\vec{x}}_n)_n$ such that for any $\zeta \in [\delta, \Delta]$,
\begin{align*}
\lim_{n\rightarrow \infty}\frac{\pi(\tilde{\vec{x}}_n)}
{\pi(\tilde{\vec{x}}_n-\operatorname{sign}(\tilde{\vec{x}}_n)\zeta)} = 0, \text{ and }
\lim_{n\rightarrow \infty}\frac{\pi(\tilde{\vec{x}}_n+\operatorname{sign}(\tilde{\vec{x}}_n)\zeta)}
{\pi(\tilde{\vec{x}}_n)} = 0.
\end{align*}
\end{assumption}

\begin{theorem}[Ergodicity of adaptive MP-MCMC]
\label{thm:ergodicity_adaptive_mpmcmc_positive}
Under the conditions of Assumption \ref{assumption:continuity_measure},
\ref{assumption:intgrability_dim_adapt} and 
\ref{assumption:tail_convergence_dim_adapt}, and if $\mathcal{Y}$ is
bounded, the adaptive MP-MCMC method described by 
\ref{algorithm:adaptive_mp_mcmc} is ergodic.
\begin{proof}
For a proof, which is again based on Theorem \ref{thm:theorem2roberts2007}, 
we refer to Appendix \ref{subsec:ergodicity_adapt_mpmcmc_positive}.
\end{proof}
\end{theorem}






















Containment: In order to show this we will make use of Corollary 2 of 
\cite{bai2011containment}, which states sufficient conditions under which
the containment condition holds true:

\begin{theorem}[Corollary 2 of \cite{bai2011containment}]
Consider the family of $\{{P}_\gamma: \gamma \in \mathcal{Y}\}$ of 
Markov chains on $\Omega^M \subset \mathbb{R}^{Md}$, satisfying the following conditions:
\begin{enumerate}[label=\arabic*)]
\item for any compact $C\in \mathcal{B}(\Omega^M)$, there exists $m\in \mathbb{N}$, $\delta>0$ and a probability measure $\nu_\gamma$ on $C$ such that 
\begin{align*}
{P}_\gamma^m(\vec{z},\cdot)\ge \delta \nu_\gamma(\cdot) \quad \text{for all $\vec{z}\in C$, 
$\gamma \in \mathcal{Y}$}, 
\text{ and},
\end{align*}
\item there is a function $V:\Omega^M\rightarrow(1,\infty)$ such that for any compact 
$C\in \mathcal{B}(\Omega^M)$, we have $\sup_{\vec{z}\in C}V(\vec{z}) <\infty$, 
$p(V)< \infty$ \tobi{check whether the latter is actually the condition we need - 
might be integral over $\pi$ instead. Or is it possible to adapt Corollary directly
to full joint distribution $p$ on the space of accepted samples?} and
\begin{align*}
\limsup_{|\vec{z}|\rightarrow \infty}\sup_{\gamma \in \mathcal{Y}} \frac{{P}_\gamma V(\vec{z})}{V(\vec{z})}<1,
\end{align*}
\end{enumerate}
then for any adaptive strategy using $\{{P}_\gamma: \gamma \in \mathcal{Y} \}$, 
containment holds.
\end{theorem}

%According to Theorem \ref{thm:theorem3bai2011}, containment is implied if the 
%underlying family of transition kernels is S.G.E.. 


%It was proven in \cite{roberts2007coupling} that simultaneous strongly aperiodic 
%geometric ergodicity implies containment, which we will use in what follows. 

%\vspace{2cm}

%A family of transition kernels $\{P_\gamma: \gamma \in \mathcal{Y} \}$ is simultaneous 
%strongly aperiodic 
%geometric ergodic (S.S.A.G.E.) if there is $C \in \mathcal{B}(\mathcal{Z})$, a function $V:\mathcal{Z}\rightarrow[1,\infty)$ and $\lambda<1$, $b<\infty$
%such that $\sup_{z\in C}V(z) < \infty$, and
%\begin{itemize}
%\item $\forall \ \gamma\in \mathcal{Y}\ \exists$ a probability measure $\nu_\gamma$ on $C$ such that $P_\gamma(z,\cdot)\ge \delta \nu_\gamma(\cdot)$ for all $z\in C$, and
%\item $P_\gamma V(z) \le \lambda V(z) + b \mathbbm{1}_C(z)$ for all $\gamma\in \mathcal{Y}, z\in\mathcal{Z}$,
%\end{itemize}
%where $P_\gamma V(z) := \mathbb{E}[V(Z_1)|Z_0=z]$.

%\vspace{2cm}
Considering 1): find $\delta>0$ and $\nu_\gamma$ such that 
${P}_\gamma (\vec{z}, B) \ge \delta \nu_\gamma(B)$ 
for all $B\in \mathcal{B}(C)$ and for all $\vec{z}\in C, \gamma \in \mathcal{Y}$, 
where $C=C_{1:M}\in \mathcal{B}(\Omega^M)$ is an arbitrary compact set. Let
\begin{align*}
\tilde{C} = \bigcup_{m=1}^M C_m.
\end{align*}
Clearly, $\tilde{C}$ is compact. Since $\pi$ is assumed to be continuous and 
positive, and since $\mathcal{Y}$ is bounded, there is a $c_A>0$ such that
%there are
%$\hat{\vec{y}}_1, ..., \hat{\vec{y}}_{N+1} \in \tilde{C}$ and 
%$\hat{\gamma} \in \overline{\mathcal{Y}}$ such that
\begin{comment}
\begin{align}
c_A := \frac{\pi(\hat{\vec{y}}_i)N_{\hat{\gamma}} (\hat{\vec{y}}_{i}, \hat{\vec{y}}_{\setminus{i}}) }
{\sum_{j=1}^{N+1}\pi(\hat{\vec{y}}_j)N_{\hat{\gamma}} (\hat{\vec{y}}_{j}, \hat{\vec{y}}_{\setminus{j}})} 
\le \frac{\pi({\vec{y}}_i)N_{{\gamma}} ({\vec{y}}_{i}, {\vec{y}}_{\setminus{i}}) }
{\sum_{j=1}^{N+1}\pi({\vec{y}}_j)N_{{\gamma}} ({\vec{y}}_{j}, {\vec{y}}_{\setminus{j}})} 
\end{align}
\end{comment}
\begin{align}
c_A \le \frac{\pi({\vec{y}}_i)N_{{\gamma}} ({\vec{y}}_{i}, {\vec{y}}_{\setminus{i}}) }
{\sum_{j=1}^{N+1}\pi({\vec{y}}_j)N_{{\gamma}} ({\vec{y}}_{j}, {\vec{y}}_{\setminus{j}})}, 
\label{eq:boundness_finite_chain_transition_probability}
\end{align}
for all $\vec{y}_{1}, ..., \vec{y}_{N+1} \in \tilde{C}$ and all 
$\gamma \in \mathcal{Y}$. 
%Similarly, there are 
%$\tilde{\vec{y}}_1, ..., \tilde{\vec{y}}_{N+1} \in \tilde{C}$ and a 
%$\tilde{\gamma} \in \overline{\mathcal{Y}}$,
Similarly, there is a $c_N>0$ such that
\begin{align*}
c_N \le N_\gamma ({\vec{y}}_{i}, {\vec{y}}_{\setminus{i}}),
\end{align*}
\begin{comment}
\begin{align}
0 < c_N := N_{\tilde{\gamma}} (\tilde{\vec{y}}_{i}, \tilde{\vec{y}}_{\setminus{i}})
\le N_\gamma ({\vec{y}}_{i}, {\vec{y}}_{\setminus{i}}),
\end{align}
\end{comment}
for all $\vec{y}_{1}, ..., \vec{y}_{N+1} \in \tilde{C}$ and all 
$\gamma \in \mathcal{Y}$.
\begin{comment}
Since the Gaussian proposal kernel is symmetric, the acceptance ratio reduces to $R(y,y') = \frac{1}{N} \min(1, \pi(y')/\pi(y))$. Further,
due to Assumption \ref{assumption:continuity_measure}, $R$ is continuous.
Therefore, there is $\hat{y}, \hat{y}' \in [0,1]^d$ such that
\begin{align}
\hat{R} := R(\hat{y}, \hat{y}') = \min_{y,y' \in [0,1]^d}R(y, y').
\end{align}
Similarly, there is $\hat{\gamma} \in \Gamma$ and $\tilde{y}, \tilde{y}'\in [0,1]^{d}$ such that
\begin{align}
\hat{N} := N_{\hat{\gamma}}(\tilde{y}, \tilde{y}') = \min_{y, y'\in [0,1]^{d}} N_\gamma(y, y') \quad \forall \ \gamma \in \Gamma,
\end{align}
where we used that $\Gamma$ is bounded.
\end{comment}
Without loss of generality, let $i_0=1$ and thus $\vec{x}_M=\vec{y}_{1}$. 
Further, let ${i}_1, ..., {i}_M\in \{2,...,N+1\}$ be chosen fixed.
%such 
%that $i_m \neq i_{m-1}$ for all $m=1,...,M$ \tobi{why need this second
%condition again?}. 
With $S_{i_m}(B)$ as defined 
in \eqref{eq:Sim_set}, we have,
%\tobi{Among the actual values of $(y^0_{1:N+1}, I_{1:M}^0=i^0_{1:M})$, only
%$y^0_{I_M}=x$ matters, i.e.\ indeed transition kernel only depends on $x$ - need
%for more appropriate notation, see above?}
\begin{align}
{P}(\vec{z}, B) &\ge P\Big(\vec{x}_M, \bigcap_{m=1}^M S_{i_m}(B)\Big)
\\
&= \int_{\bigcap_m {T_{i_m}(B)}}
N_{\gamma}(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}}) 
\prod_{m=1}^M A({i_{m-1}}, {{i_m}})
\mathrm{d}\vec{y}_{\setminus{i_0}}\nonumber\\
&\ge c_A^M \int_{\bigcap_m {T_{i_m}(B)}}
N_\gamma (\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}})
\mathrm{d}\vec{y}_{\setminus{i_0}}\nonumber\\
& \ge c_A^M c_N \lambda\left(\bigcap_m T_{i_m}(B)\right)\nonumber\\
& = \delta \nu(B),\nonumber
\end{align}
where $\delta := c_A^M c_N>0$, $\nu(B):=\lambda(\bigcap_m T_{i_m}(B))$, 
%\tobi{Where is $T_{i_m}(B)$ defined?}
and $\lambda(\cdot)$ denotes the Lebesgue measure, which concludes
the proof of 1).\\

%Let $V\equiv 1 on \mathcal{Z}$ and let $C=\mathcal{Z}$. Clearly, $P_\gamma V(z) = 1$, thus
%the second item is fulfilled for $\lambda=1/2$ and $b=1$. Further, for any $B\in \mathcal{Z}$
%let $K\in \mathcal{B}(\mathbb{R}^{Nd})$, compact.

%\begin{align}
%P_\gamma(z, B) &= \int_{\{ y_{\setminus{I_M^{\operatorname{old}}}}: y_{1:N+1}\in B_y \} 
%\times B_I} \prod_{i\neq %I_M^{\operatorname{old}}}N(y_{I_M^{\operatorname{old}}}, y_i) \prod_{m=1}^M A(I_{m-1}, I_m| y_{1:N+1})\mathrm{d}y_{\setminus{I_M^{\operatorname{old}}}}\mathrm{d}I_{1:M}\\
%&\ge \int_{\{ y_{\setminus{I_M^{\operatorname{old}}}}: y_{1:N+1}\in B_y \}\cap K \times B_I} N_{\min} 
%\end{align}


%\vspace{3cm}


\tobi{Note that in the following you have used the definition of Peskun
transition probabilities on the finite state chain, i.e.\ the one
introduced in \cite{calderhead2014general}, instead of the one we should
have used, which is the stationary transition probability on the
finite state chain and which has been used all over the place and in
particular in the first part of this proof, that is, 1). - FIX THIS!\\

This problem can in general NOT be solved by argueing that Peskun 
acceptance probability is at least as high as the stationary distribution
of the auxiliary variable. This is only true for the case $M=N=1$.

All in all, the 2) part of this proof is a big mess and I need some
serious support for finishing this proof!}


Considering 2): show that if $V(\vec{x}_{1:M}):= c(s)\pi(\vec{x}_1)^{-s}$ 
for all $\vec{x}_{1:M} \in \Omega^M$, and for some
$c(s)>1$ and some $s\in (0,1)$, then for any compact $C\in \mathcal{B}(\Omega^M)$, 
we have $\sup_{\vec{x}_{1:M}\in C}V(\vec{x}_{1:M}) <\infty$, 
$\int \pi(\vec{x})^{1-s}\mathrm{d}\vec{x}< \infty$, and
\begin{align}
\limsup_{|\vec{x}_{1:M}|\rightarrow \infty}\sup_{\gamma \in \Gamma} \frac{\tilde{P}_\gamma V(\vec{x}_{1:M})}{V(\vec{x}_{1:M})}<1.
\label{eq:converge_condition_dim_adapt}
\end{align}

Since the target is continuous, obviously $\sup_{\vec{x}_{1:M}\in C}V(\vec{x}) <\infty$ 
is satisfied, and $\int \pi(\vec{x})^{1-s}\mathrm{d}\vec{x}< \infty$ holds true by
assumption \ref{assumption:intgrability_dim_adapt}. As $\pi$ is continuous and integrable 
over $\Omega$, it holds $c(s):= 1+ \sup_{\vec{x}} \pi(\vec{x})^s <\infty$ and thus, 
$V(\vec{x}_{1:M})> 1$ for all $\vec{x}_{1:M} \in \Omega^M$.\\

To prove \eqref{eq:converge_condition_dim_adapt}, let us first
consider the special case $M=N=1$, which corresponds to usual Metropolis-Hastings. 
Let $R(\vec{x}):= \{\vec{z}=\vec{x}+\vec{\zeta}: \pi(\vec{z})< \pi(\vec{x})\}$ and 
$A(\vec{x}):=\{\vec{z}=\vec{x}+\vec{\zeta}: \pi(\vec{z})\ge \pi(\vec{x})\}$. Thus, 
points in $A(\vec{x})\subset \mathbb{R}^d$ are always accepted while points in 
$R(\vec{x})\subset \mathbb{R}^d$ have positive probability of being rejected.
Using $\vec{y}_{i_0}=\vec{x}$, we have
\begin{align*}
\frac{\tilde{P}_\gamma V(\vec{x})}{V(\vec{x})}
&= \int_{R(\vec{x})} N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}}) \left[ 1- \frac{\pi(\vec{y}_{\setminus{i_0}})}{\pi(\vec{y}_{i_0})}\right] \mathrm{d}\vec{y}_{\setminus{i_0}} \\
&\quad + \int_{R(\vec{x})} N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}})\frac{\pi(\vec{y}_{\setminus{i_0}})}{\pi(\vec{y}_{i_0})} \left(\frac{\pi(\vec{y}_{\setminus{i_0}})}{\pi(\vec{y}_{i_0})}\right)^{-s} \mathrm{d}\vec{y}_{\setminus{i_0}} \\
&\quad +\int_{A(\vec{x})} N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}})\left(\frac{\pi(\vec{y}_{\setminus{i_0}})}{\pi(\vec{y}_{i_0})}\right)^{-s} \mathrm{d}\vec{y}_{\setminus{i_0}}\\
&= \int_{\mathbb{R}^d}N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}}) \eta( \vec{y}_{\setminus{i_0}})\mathrm{d}\vec{y}_{\setminus{i_0}},
\end{align*}
where
\begin{align*}
\eta(\vec{y}_{\setminus{i_0}})= 
\begin{cases} 1-\frac{\pi(\vec{y}_{\setminus{i_0}})}{\pi(\vec{y}_{i_0}} + \left(\frac{\pi(\vec{y}_{\setminus{i_0}})}{\pi(\vec{y}_{i_0})}\right)^{1-s}  &\mbox{if } \vec{y}_{\setminus{i_0}}\in R(\vec{x}) \\
\left(\frac{\pi(\vec{y}_{i_0})}{\pi(\vec{y}_{\setminus{i_0}})}\right)^{s}  & \mbox{if } \vec{y}_{\setminus{i_0}}\in A(\vec{x}) \end{cases}.
\end{align*}
Clearly, $\eta(\vec{y}_{\setminus{i_0}})=(\pi(\vec{y}_{i_0})/\pi(\vec{y}_{\setminus{i_0}}))^{s}\le 1$ on $A(\vec{x})$ by definition. By setting 
$w:=\pi(\vec{y}_{\setminus{i_0}})/\pi(\vec{y}_{i_0})$, we have that 
$\eta(\vec{y}_{\setminus{i_0}})=1-w+w^{1-s}$ on $R(\vec{x})$ with $w \in [0,1]$. Maximising this term leads to $w=(1-s)^{1/s}$ and $\eta(\vec{y}_{\setminus{i_0}}) \le 1 + (1-s)^{(1-d)/d}$ on $R(\vec{x})$. Therefore,
\begin{align*}
\frac{\tilde{P}_\gamma V(\vec{x})}{V(\vec{x})} \le 1 + (1-s)^{(1-d)/d}.
\end{align*}
The rest of the proof follows analogously to the proof of Theorem 5.5 in
\cite{latuszynski2013adaptive}, which requires an additional assumption upon the target (Assumption 5.4 in \cite{latuszynski2013adaptive}). Since
$\Gamma$ is bounded and $N_\gamma$ is a continuous density, 
there exist $0< \delta < \Delta \le \infty$ such that
\begin{align*}
\beta := \inf_{\gamma \in \Gamma} \int_{\delta}^{\Delta} N_\gamma(\vec{x})\mathrm{d}\vec{x} >0,
\end{align*}
where $N_\gamma$ here denotes the Normal density defined as a function of
the difference between mean and evaluation point. Further, due
to Assumption \ref{assumption:tail_convergence_dim_adapt}, 
Assumption 5.4 in \cite{latuszynski2013adaptive} is satisfied. This 
concludes the proof of the case $N=M=1$.\\

Let us consider the general case, i.e.\ $N, M\in \mathbb{N}$. In every iteration, $N$ new proposals $\vec{y}_{\setminus{i_0}}$ are generated. For the first accepted sample being equal to, say, the $\ell$th of those
new proposals, i.e.\ $\vec{y}_{i_1}=\vec{y}_{\setminus{i_0}, \ell}$ there exist two cases:
first, $\vec{y}_{\setminus{i_0}, \ell} \in R(\vec{x})$, and second, 
$\vec{y}_{\setminus{i_0}, \ell} \in A(\vec{x})$. For the first accepted sample being equal to the previous sample, i.e.\ $\vec{y}_{i_1}=\vec{y}_{i_0}$, at least one of the $N$ new proposals
needs to belong to $R(\vec{x})$, since otherwise, 
$P(\text{accept } \vec{y}_{i_0} \text{ as $1$st sample}) = 1-\sum_{\ell=1}^N A(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}, \ell})= 0$. Without loss of generality,
we may say $\vec{y}_{\setminus{i_0},1}\in R(\vec{x})$ in this case. Using the notation,
\begin{align*}
R_\ell(\vec{x}) &= \mathbb{R}^{d(\ell -1)}\times R(\vec{x}) \times \mathbb{R}^{d(N-\ell)},
\text{ and,}\\
A_\ell(\vec{x}) &= \mathbb{R}^{d(\ell -1)}\times A(\vec{x}) \times \mathbb{R}^{d(N-\ell)},
\end{align*}
the previous considerations lead to\\


\tobi{There two things wrong below: one is that in the acceptance probability the 
proposal kernel terms are missing. Second is that $V$ is defined to have a value
depending on the first accepted sample, but below we're using 
$V(\vec{x})=f(\vec{y}_{i_0})$, which says that $V$ depends on the last accepted
sample in one iteration. Note that $\vec{x}\in \mathbb{R}^{Md}$.}
\\


\begin{align*}
\frac{\tilde{P}_\gamma V(\vec{x})}{V(\vec{x})} 
&= \int_{\mathbb{R}^{Nd}} N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}})
\sum_{i_1, ..., i_M=1}^{N+1} \prod_{j=1}^M A(\vec{y}_{i_{j-1}}, \vec{y}_{i_j})
\frac{V(\vec{y}_{i_1})}{V(\vec{y}_{i_0})} \mathrm{d}\vec{y}_{\setminus{i_0}}\\
&= \sum_{\ell=1}^{N} \int_{R_\ell(\vec{x})}N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}})
\mathbbm{1}({\vec{y}_{i_1}=\vec{y}_{\setminus{i_0},\ell}})
\frac{1}{N} \frac{\pi(\vec{y}_{\setminus{i_0}, \ell})}{\pi(\vec{y}_{i_0})} \left( \frac{\pi(\vec{y}_{\setminus{i_0},\ell})}{\pi(\vec{y}_{i_0})} \right)^{-s}
\sum_{i_2, ..., i_M=1}^{N+1} \prod_{j=2}^M A(\vec{y}_{i_{j-1}}, \vec{y}_{i_j})
\mathrm{d}\vec{y}_{\setminus{i_0}}\\
&\quad +\sum_{\ell=1}^{N} \int_{A_\ell(\vec{x})}N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}})
\mathbbm{1}({\vec{y}_{i_1}=\vec{y}_{\setminus{i_0},\ell}})
\frac{1}{N} \cdot 1 \cdot
\left(\frac{\pi(\vec{y}_{\setminus{i_0}, \ell})}{\pi(\vec{y}_{i_0})}\right)^{-s}
\sum_{i_2, ..., i_M=1}^{N+1} \prod_{j=2}^M A(\vec{y}_{i_{j-1}}, \vec{y}_{i_j})
\mathrm{d}\vec{y}_{\setminus{i_0}}\\
&\quad + \int_{R_1(\vec{x})}N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}})
\mathbbm{1}({\vec{y}_{i_1}=\vec{y}_{{i_0}}})
\left[ 1-\sum_{\ell =1}^N A(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0},\ell})\right]
\cdot 1 \cdot 
\sum_{i_2, ..., i_M=1}^{N+1} \prod_{j=2}^M A(\vec{y}_{i_{j-1}}, \vec{y}_{i_j})
\mathrm{d}\vec{y}_{\setminus{i_0}}\\
&= \int_{\mathbb{R}^{Nd}} N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}})
\Bigg\{
\frac{1}{N} \sum_{\ell=1}^N \mathbbm{1}({\vec{y}_{i_1}=\vec{y}_{\setminus{i_0},\ell}})
\mathbbm{1}(\vec{y}_{\setminus{i_0}} \in R_\ell(\vec{x}))
\left( \frac{\pi(\vec{y}_{\setminus{i_0},\ell})}{\pi(\vec{y}_{i_0})} \right)^{1-s}\\
&\quad\quad\quad +
\mathbbm{1}({\vec{y}_{i_1}=\vec{y}_{{i_0}}}) 
\mathbbm{1}(\vec{y}_{\setminus{i_0}} \in R_1(\vec{x}))
\left[ 1-\sum_{\ell =1}^N A(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0},\ell})\right]\\
&\quad\quad\quad +
\frac{1}{N} \sum_{\ell=1}^N \mathbbm{1}({\vec{y}_{i_1}=\vec{y}_{\setminus{i_0},\ell}})
\mathbbm{1}(\vec{y}_{\setminus{i_0}} \in A_\ell(\vec{x}))
\left( \frac{\pi(\vec{y}_{\setminus{i_0},\ell})}{\pi(\vec{y}_{i_0})} \right)^{-s}
\Bigg\}
\sum_{i_2, ..., i_M=1}^{N+1} \prod_{j=2}^M A(\vec{y}_{i_{j-1}}, \vec{y}_{i_j})
\mathrm{d}\vec{y}_{\setminus{i_0}}\\
&= \int_{\mathbb{R}^{Nd}} N_\gamma(\vec{y}_{i_0}, \vec{y}_{\setminus{i_0}})
\eta(\vec{y}_{1:N+1})\sum_{i_2, ..., i_M=1}^{N+1} \prod_{j=2}^M A(\vec{y}_{i_{j-1}}, \vec{y}_{i_j})
\mathrm{d}\vec{y}_{\setminus{i_0}},
\end{align*} 
where $\eta(\vec{y}_{1:N+1})$ is defined suitably as the term inside
the curly brackets above. Since $(\pi(\vec{y}_{\setminus{i_0},\ell})/\pi(\vec{y}_{i_0}))^{-s}\le 1$
for any $\vec{y}_{\setminus{i_0}}\in A_\ell(\vec{x})$, it holds
\tobi{Hm, the following estimate might not be quite right...}
\begin{align*}
\eta(\vec{y}_{1:N+1}) \le \max_{w_\ell \in [0,1]}
\left(  
\frac{1}{N}\sum_{\ell=1}^N w_\ell^{1-s} + 
\left[
1- \frac{1}{N}\sum_{\ell=1}^N w_\ell 
\right]
\right).
\end{align*}
The maximum value is achieved by $w_\ell = (1-s)^{1/s}$, which leads to
$\eta(\vec{y}_{1:N+1}) \le 1 + (1-s)^{(1-s)/s}$, and therefore 
\begin{align*}
\frac{\tilde{P}_\gamma V(\vec{x})}{V(\vec{x})} \le 1 + (1-s)^{(1-d)/d}.
\end{align*}
The rest of the proof follows similarly to the $N=M=1$ case considered above.
\tobi{Verify the proof above: first, verify the correctness of applying the 
Theorem 5.5 from \cite{latuszynski2013adaptive} - note that they considered
adaptivity in the context of Gibbs samplers only. Second, verify the 
calculations for the $N=$general, $M=$general case.}
